Asymptotics in an Asymptotic CFT

In this work we illustrate the resurgent structure of the $\lambda$-deformation; a two-dimensional integrable quantum field theory that has an RG flow with an $SU(N)_k$ Wess-Zumino-Witten conformal fixed point in the UV. To do so we use modern matched asymptotic techniques applied to the thermodynamic Bethe ansatz formulation to compute the free energy to 38 perturbative orders in an expansion of large applied chemical potential. We find numerical evidence for factorial asymptotic behaviour with both alternating and non-alternating character which we match to an analytic expression. A curiosity of the system is that it exhibits the Cheshire Cat phenomenon with the leading non-alternating factorial growth vanishing when $k$ divides $N$. The ambiguities associated to Borel resummation of this series are suggestive of non-perturbative contributions. This is verified with an analytic study of the TBA system demonstrating a cancellation between perturbative and non-perturbative ambiguities.

==> Sections/04_Perturbative.tex <==
%\section{Perturbative Results } \label{sec:PertTBA}

%%%% NOTHING IN THIS SECTION %%%%%

==> Sections/A_WH.tex <==
\section{Wiener Hopf Techniques } \label{ap:WH}
The derivation in this Section is not new \cite{hasenfratz1990exact1,hasenfratz1990exact2,Forgacs:1991rs,Balog:1992cm}, but serves to flesh out some of the steps motivating our transformed integral Equations. We will be starting form the ``free energy TBA" system, which was related to the ``total energy TBA" system. For $\theta \in I= [-B, B]$, we have that $\epsilon(\theta)$ is determined by the equations
\begin{equation}
\begin{split} 
    &\epsilon(\theta) - \int_{-B}^B d\theta' K(\theta -\theta') \epsilon(\theta') =   h -m \cosh \theta \\ 
    & \Delta F(h) = F(h) - F(h=0) = -\frac{m}{2\pi} \int_{-B}^B d \theta \cosh (\theta) \epsilon( \theta)  \\
     &\epsilon(\pm B) = 0\,.
\end{split}      
\end{equation}

It is convenient to analyse this system in Fourier space\footnote{We use the Fourier transform conventions
\begin{equation*}
   \tilde{f}(\omega)  = \int_{-\infty}^{\infty} d\theta e^{i \omega \theta} f(\theta) \, . 
\end{equation*}} where Wiener-Hopf factorisation techniques can be deployed \cite{hasenfratz1990exact1,hasenfratz1990exact2,Forgacs:1991rs,Balog:1992cm}. To perform the Fourier transform we need to extend the limits on the convolution integral to $\pm \infty$ which we do by first letting $\epsilon(\theta)$ extend to the zero function outside of $I=[-B,B]$.%\footnote{This is not unlike the function $\epsilon^+(\theta)$ which appears in Appendix \ref{ap:FreeEnergy}.}  
To soak up the remaining contributions of the convolution outside of this domain we let  
\begin{equation}
    \epsilon(\theta) - \int_{-\infty}^\infty d\theta' K(\theta -\theta') \epsilon(\theta') =  g(\theta) + Y(\theta- B) + Y(-\theta - B)\,,
\end{equation}
now valid for $\theta \in \mathbb{R}$ with  $Y$ unknown and $g(\theta)$ chosen such that it agrees with $h -m \cosh \theta $ on $I$.    This can now be Fourier transformed 
\begin{equation}\label{eq:FT1}
    \frac{1}{G_+(\omega) G_-(\omega)} \tilde{\epsilon }(\omega) = \tilde{g}(\omega) + e^{i\omega B } \tilde{Y}(\omega) + e^{-i \omega B} \tilde{Y}(-\omega)\,,
\end{equation}
in which we used the Wiener-Hopf factorisation of the kernel 
\begin{equation}
  1-K(\omega)   = \frac{1}{G_+(\omega)G_-(\omega)}\,,
\end{equation}
where   $G_+ $  is analytic in the UHP, $G_-$ analytic in the LHP and  $G_-(\omega)=G_+(-\omega)$  is assumed.   In what follows for a function $f(\omega)$ we define its analytic projections into the UHP and LHP as 
\begin{equation}
    [f]_\pm = \pm  \frac{1}{2\pi i }\int_{-\infty}^\infty d\omega' \frac{f(\omega')}{\omega' - \omega \mp i \delta }\,,
\end{equation}
such that $f = [f]_+ + [f]_-$ and $[ [f]_+ ]_- = 0 $ and $[ [f]_+ ]_+ = [f]_+$. Furthermore, it is useful to employ the definitions 
\begin{equation}
    g_\pm(\omega)  = e^{\pm i B \omega} \tilde{g}(\omega) \, , \quad \epsilon_\pm(\omega)  = e^{\pm i B \omega} \tilde{\epsilon}(\omega)\, ,\quad  \sigma(\omega) = \frac{G_-(\omega)}{G_+(\omega) }\,,
\end{equation}
 \begin{equation}
Q_+(\omega) = G_+(\omega) \tilde{Y}(\omega) \, , \quad Q_-(\omega) = Q_+(-\omega)= G_-(\omega) \tilde{Y}(-\omega) \,.
\end{equation}

We now take the equation \eqref{eq:FT1} and multiply by $e^{i \omega B} G_-(\omega)$ to give
\begin{equation}\label{eq:FT2}
\begin{aligned}
        \frac{1}{G_+(\omega)  } \epsilon_+(\omega) &=G_-(\omega) g_+ (\omega) + e^{2 i\omega B } G_-(\omega) \tilde{Y}(\omega) +    G_-(\omega)\tilde{Y}(-\omega) \\
        &=G_-(\omega) g_+ (\omega) + e^{2 i\omega B } \sigma(\omega) Q_+(\omega)+ Q_-(\omega) \,.
\end{aligned}
\end{equation}
Taking the WH projections yields two equations: 
\begin{eqnarray}
&0 = [G_- g_+]_- + [e^{2 i\omega B } \sigma Q_+]_- + Q_-\,, \\ 
&\frac{\epsilon_+}{G_+} = [G_- g_+]_+ + [e^{2 i\omega B } \sigma Q_+]_+ \,.
\end{eqnarray}
The first can be solved for $Q$ (in principle, but of course not in general in closed form), which seeds the second equation to determine $\epsilon_+(\omega)$ and hence   the free energy at finite density\footnote{infinite volume and zero temperature.}. 
The relation between $B$ and $h$ is determined by the boundary conditions that $\epsilon(\pm B)=0$.


In the case where $G_+(0)$ is finite the analysis can be further streamlined by   rephrasing  eq. \eqref{eq:FT1} as 
\begin{equation}\label{eq:FT1bis} 
    \tilde{\epsilon }(\omega) =  e^{i\omega B } \tilde{V}(\omega) G_-(\omega)    + e^{-i \omega B}  \tilde{V}(-\omega)  G_+(\omega)  \, . 
\end{equation}
 This is achieved by  making using of the explicit form  
\begin{equation}
\tilde{g} (\omega)  =  e^{i B \omega} \left( -\frac{i h}{\omega} + \frac{i m e^B}{2} \frac{1}{\omega - i}  \right)  + e^{-i B \omega} \left(\frac{i h}{\omega} -\frac{i m e^B}{2} \frac{1}{\omega + i}   \right)    \,.
\end{equation}
 to relate $\tilde{V}(\omega) $ and $\tilde{Y}(\omega) $ as   
\begin{equation}
 \tilde{V}(\omega)   = G_+(\omega) \left( \tilde{Y}(\omega) - \frac{h i }{\omega } - \frac{i m e^B}{2 }\frac{1}{i-\omega} \right) \, . 
\end{equation}
 This implies in particular that   $\tilde{V}(\omega)$ is not analytic in UHP, instead it has poles at $\omega =i $ and $\omega = i 0$. Consequently, $[\tilde{V}(-\omega)]_- \neq \tilde{V}(-\omega)$ but rather 
\begin{equation}
 [\tilde{V}(-\omega)]_- = \tilde{V}(-\omega) +  \frac{h i G_-(0) }{\omega + i \delta } - \frac{i m e^B G_+(i) }{2} \frac{1}{\omega + i} \, .
\end{equation}
 We could proceed to carry out the WH evaluation directly in terms of this function $\tilde{V}$, however it is more elegant to remove the pole at $\omega = i $ by defining $\tilde{U}(\omega) = (1+ i \omega) \tilde{V}(\omega)$.  Multiplying eq.\eqref{eq:FT1bis}  by $ (1- i \omega) e^{i B \omega} / G_+(\omega)$ yields 
 \begin{equation}
     (1-i\omega) \frac{ \epsilon_+(\omega) }{G_+(\omega) }=  e^{2 i\omega B } \tilde{U}(\omega) \varrho(\omega)      +    \tilde{U}(-\omega)    \, . 
\end{equation}
in which
\begin{equation} \label{eq:varrhodefn}
\varrho(\omega) = \frac{ 1-i\omega} {   1+i\omega} \frac{G_-(\omega) }{G_+(\omega) }  \, . 
\end{equation}

Now the WH projections read 
\begin{equation}\label{eq:FT1bisWH} 
\begin{aligned}
  0 &= [e^{2 i\omega B } \tilde{U}(\omega) \varrho(\omega)   ]_- + \tilde{U}(-\omega) + \frac{ih G_-(0) }{\omega+ i\delta } \\ 
 (1-i\omega) \frac{ \epsilon_+(\omega) }{G_+(\omega) } &=  [e^{2 i\omega B } \tilde{U}(\omega) \varrho(\omega)   ]_+ - \frac{ih G_-(0) }{\omega+ i\delta } \, .  
\end{aligned}
\end{equation}
We further refine by rescaling $ \tilde{U}(\omega) = h G_-(0) u(\omega)   $ so that we arrive at the integral equation which is the main subject of Section \ref{sec:transseries}:
\begin{equation}
 u(\omega)  =   \frac{i  }{\omega- i\delta }  + \frac{1}{2 \pi i} \int d\omega' \frac{e^{2 i\omega' B } u(\omega') \varrho(\omega')    }{\omega'+\omega + i \delta } 
\end{equation}
From the second of Equation \eqref{eq:FT1bisWH} we have 
$$ (1-i\omega) \frac{ \epsilon_+(\omega) }{G_+(\omega) }   =  + h G_-(0)  \frac{1}{2\pi i} \int d\omega' \frac{1}{\omega' - \omega - i \delta}  e^{2 i\omega' B } u(\omega') \varrho(\omega')   - \frac{ih G_-(0) }{\omega+ i\delta } \,.$$
Evaluating this at $\omega=i$ gives
$$  \epsilon_+(i)     = \frac{ h}{2} G_+(i) G_-(0)  \left( 1 -   \frac{1}{2\pi i} \int d\omega' \frac{1}{\omega' -i}  e^{2 i\omega' B } u(\omega') \varrho(\omega')  \right) \,.    $$
We can therefore compute the free energy 
\begin{equation} \label{eq:freeenergyinu3}
\begin{split}
    \Delta F(h) &=   - \frac{1}{2\pi}m e^B   \epsilon_+(i) \\
        &=   -\frac{1}{2\pi}  h^2 u(i) G_-(0)^2   \left( 1 -   \frac{1}{2\pi i} \int_{-\infty}^\infty d\omega' \frac{e^{2 i\omega' B } u(\omega') \varrho(\omega')}{\omega' -i}    \right)  \,,
\end{split}
\end{equation}
in the last step we invoked that the boundary condition $\epsilon(\pm B) =0$ can be reformulated as
\begin{equation} \label{eq:u(i)bc2}
    u(i) = \frac{m}{2 h} e^{B} \frac{G_+(i) } {G_+(0)}\,.
\end{equation}

% This results in 
%   \begin{equation} \label{eq:IRFinu}
%   \begin{split}
%  \mathcal{F}(h) =& - \frac{h^2}{2\pi} u(i) G_+(0)^2 \left[ 1- \frac{1}{2 \pi i} \int_{C_\pm} \frac{e^{-2 B x'} \delta \varrho(i x') u(i x') }{x' -1} dx'\right.  \\
%  \quad -\left. e^{-2B}\varrho(i \pm \epsilon) u(i) - \sum_{n\geq 1} \frac{e^{-2 B x_n}\varrho_{n, \pm} u_n}{x_n-1} \right]  \\
%    \Delta F (h) =&- \frac{h^2}{2\pi} u(i) G_+(0)^2 \bigg(  1 + \frac{v^2}{\pi} \int \frac{e^{-\eta} P(\eta,v)u(\eta)}{\eta v-1}  d\eta  \\&- e^{-2B}\varrho(i \pm \epsilon) u(i) - \sum_{n\geq1} \frac{q^n \varrho_{n, \pm} u_n}{\mu n-1} \bigg)
%   \end{split}
%  \end{equation}
